Diffeomorphic Shape Matching by Operator Splitting in 3D Cardiology Imaging

We develop an operator splitting approach to solve diffeomorphic matching problems for sequences of surfaces in three-dimensional space. The goal is to smoothly match, at a very fast rate, finite sequences of observed 3D-snapshots extracted from movies recording the smooth dynamic deformations of "soft" surfaces. We have implemented our algorithms in a proprietary software installed at The Methodist Hospital (Cardiology) to monitor mitral valve strain through computer analysis of noninvasive patients' echocardiographies.

==> makefile <==
filename=paper

compile=latexmk 


all:
	@echo ${compile} 
	${compile} -halt-on-error -pdf ${filename}.tex 
	@echo Done ....!
	open -a Skim ${filename}.pdf

paper:
	@echo ${compile} 
	${compile} -halt-on-error -pdf ${papername}.tex 
	@echo Done ....!
	@#open -a Skim ${papername}.pdf

clean:
	rm -f *.aux *.log *.dvi *.blg *.bbl \
          *.fls *.fdb_latexmk *.out     \
          *.brf *.snm *.toc *.nav       \
		  *.pdfsync *synctex.gz *.pdf
	@echo Cleaned ....! 



